Anonymity Preserving Byzantine Vector Consensus

Collecting anonymous opinions finds various applications ranging from simple whistleblowing, releasing secretive information, to complex forms of voting, where participants rank candidates by order of preferences. Unfortunately, as far as we know there is no efficient distributed solution to this problem. Previously, participants had to trust third parties, run expensive cryptographic protocols or sacrifice anonymity. In this paper, we propose a resilient-optimal solution to this problem called AVCP, which tolerates up to a third of Byzantine participants. AVCP combines traceable ring signatures to detect double votes with a reduction from vector consensus to binary consensus to ensure all valid votes are taken into account. We prove our algorithm correct and show that it preserves anonymity with at most a linear communication overhead and constant message overhead when compared to a recent consensus baseline. Finally, we demonstrate empirically that the protocol is practical by deploying it on 100 machines geo-distributed in 3 continents: America, Asia and Europe. Anonymous decisions are reached within 10 seconds with a conservative choice of traceable ring signatures.

==> arbproof/arbproof.bkp.tex <==
\section{Analysis of ARBP} \label{sec:arbproof}

% define infeasible?
% state properties or not?

In this appendix, we prove that all properties of anonymous reliable broadcast are fulfilled by our protocol, Anonymous Reliable Broadcast Protocol (ARBP) (Algorithm~\ref{alg:arb} in Section~\ref{sec:arb:arb}).

\begin{remark}
	Let $m, n, t$ be positive integers s.t. $n > 3t$. Then: \[m > \frac{n - t}{2} \Leftrightarrow m \geq \lfloor \frac{n - t}{2} + 1 \rfloor\]
\end{remark}
Thus, we refer to a process that receives some message from $\lfloor \frac{n - t}{2} \rfloor + 1$ different processes, as per the algorithm's description, as receiving that message from ``more than $\frac{n - t}{2}$'' different processes in the correctness proofs.

\begin{lemma}
\label{arb-anon}
	ARBP ensures ARB-Anonymity, which is stated as follows:
	Let $msg = (m, \sigma)$ be a message ARB-broadcast by a non-faulty process $p_i$.
	Then, it is impossible for the adversary to determine the value of $i$ with probability $Pr > \frac{1}{n - t}$.
\end{lemma}
\begin{proof}
Since the adversary $A$ can corrupt up to $t$ processes and has access to and controls their entire state, $A$ can always distinguish between their anonymous proposals.
We show that $A$ cannot determine the identity of a signer of remaining $n - t$ proposals with probability greater than randomly guessing.
We assume that an arbitrary number of executions of ARBP may take place that are each independent in the sense that input to each instance by non-faulty processes does not depend on results from any other instance.
We deal with the scenario where an instance of ARBP may depend on the result of a previous instance in AVCP (Theorem~\ref{avc-anon2}).

Let $p_i$ denote a non-faulty process that invokes $\lit{ARBP}[\ms{ID}](m)$.
$p_i$ invokes $\lit{Sign}(p_i, \ms{ID}, m)$, producing the signature $\sigma$ (line~\ref{line:arb:sign}).
Then, $p_i$ invokes ``$\lit{anon\_broadcast}$ $(\ms{ID},$\INIT$, m, \sigma)$'' (line~\ref{line:ab:initbcast}).
The adversary will eventually see the delivered message at one of its corrupted processes.
By signature anonymity and the use of anonymous channels, $A$ cannot determine $i$ with probability $Pr > \frac{1}{n - t}$.
By definition of $\lit{Sign}$, the adversary cannot produce call $\sigma' \leftarrow \lit{Sign}(p_i, \ms{ID}, m')$ for some $m'$.
Thus, by traceability and entrapment-freeness, the adversary cannot produce $(m', \sigma')$ such that $\lit{Trace}(\ms{ID}, m, \sigma, m', \sigma') \neq ``indep''$.
In particular, if $m' \neq m$, then the adversary cannot expose the identity of $p_i$ through a $\lit{Trace}$ call, as $\lit{Trace}$ will never output $i$.
Now, the adversary can only see calls of the form ``$\lit{send}$'', ``$\lit{receive}$'' or ``$\lit{anon\_receive}$'', and cannot see the computational history of non-faulty processes.
Consequently, the adversary cannot tell whether a non-faulty process has anonymously broadcast their proposal or not based on the fact that they have or have not made $\lit{send}$ calls (e.g. in broadcasting \ECHO \ messages (line~\ref{line:ab:bcastecho})).
Since the sender of an \INIT \ message propagates the corresponding \ECHO \ and \READY \ messages as if it were any other process, they cannot be de-anonymised by omission of the relevant $\lit{send}$ calls.
This holds for an arbitrary number of independent executions of ARBP.

%	We note that without anonymous channels that $p$'s index in $P$ is trivially exposed.
% frame wrt query to FindIndex
% TODO: rest of protocol (echoing etc) independent of identity of process
% can move thing about all but one echoing to this section

	% which, without considering its contents, preserves $p$'s anonymity by assumption.
%	A non-faulty process $p_i$ initially broadcasts its proposal $m$ via anonymous links (line \ref{line:ab:initbcast}), which, not considering the content of $m$, preserve the anonymity of $p_i$ by assumption.
%	Then, by TRS-Exculpability and the unforgeability of an honest process' signature, $p_i$ cannot be feasibly linked or traced to any other message, as it is non-faulty and does not double-sign, and so cannot be accused of misbehaviour.
%	Then, TRS-Anonymity ensures their identity is effectively indistinguishable from the rest of the ring.
%	We note that $f$ colluding processes can only feasibly deduce that they did not sign $m$, and so $p_i$'s identity is inexorably indistinguishable from the remaining $(n - f - 1)$ processes to them.
%	This is precisely the definition of $(n - f)$-anonymity.
%	Further, $p_i$'s subsequent participation in the protocol (the propagation of \ECHO \ and \READY \ messages) over reliable channels does not explicitly associate it with $m$.
\end{proof}
%We note that for use in multiple iterations of ARB-Broadcast, which ought to use different tags, that TRS-Anonymity guarantees that messages signed by the same signer with respect to distinct tags cannot be feasibly associated together. Thus, the protocol can be freely sequentially composed.

\begin{lemma}
\label{arb-val}
ARBP ensures ARB-Validity, which is stated as follows.
Suppose that a non-faulty process $p$ ARB-delivers $(m, \sigma)$.
Let $i = \lit{FindIndex}(\ms{ID}, m, \sigma)$ denote the output of an idealised call to $\lit{FindIndex}$.
Then if $p_i$ is non-faulty, $p_i$ must have ARB-broadcast $(m, \sigma)$.

\end{lemma}
\begin{proof}
	Let $p_i$ be non-faulty.
	From the protocol specification, $p_i$ must have invoked $\sigma \leftarrow \lit{Sign}(\ms{ID}, p_i, m)$.
	By definition of $\lit{Sign}$, no other process could have produced such a value of $\sigma$.
	By traceability and entrapment-freeness, no other process can produce a tuple $(m', \sigma')$ such that $\lit{Trace}(\ms{ID}, m, \sigma, m', \sigma') \neq$ ``indep''.
	Consequently, no process can produce a message that prevents non-faulty processes from propagating $(\ms{ID}, $\ECHO$, m, \sigma)$ messages.
	Thus, since $p_i$ is non-faulty, and therefore followed the protocol, $p_i$ ARB-broadcast $(m, \sigma)$.
\end{proof}

\begin{lemma}
\label{arb-term-1}
ARBP ensure ARB-Termination-1. That is, if a process is non-faulty and ARB-broadcasts $(m, \sigma)$, all the non-faulty processes eventually ARB-deliver $(m, \sigma)$.
\end{lemma}

\begin{proof}
	\sloppy{
	Suppose that the non-faulty process $p_i$ invokes ARBP with respect to identifier $\ms{ID}$ and message $m$.
	$p_i$ invokes ARB-broadcast, anonymously broadcasting $(\ms{ID},$\INIT$, m, \sigma)$, where $\sigma = \lit{Sign}(p_i, \ms{ID}, m)$.
	Since the network is reliable, all non-faulty processes eventually receive $(\ms{ID},$\INIT$, m, \sigma)$ (and indeed all messages broadcast by non-faulty processes).
	At line \ref{line:ab:isvalid}, $\lit{VerifySig}$ is queried with respect to $(m, \sigma)$.
	By signature correctness, $\lit{VerifySig}(\ms{ID}, m, \sigma) = 1$ is guaranteed, since $p_i$ invoked $\sigma \leftarrow \lit{Sign}(p_i, \ms{ID}, m)$.
	So, all non-faulty processes proceed to line \ref{line:ab:beginfor}.
	By traceability and entrapment-freeness, no non-faulty process could have received a message $(m', \sigma')$ such that $\lit{Trace}(\ms{ID}, m, \sigma, m', \sigma') \neq$ ``indep''.
	Consequently, all non-faulty processes reach line~\ref{line:ab:deposit} with value $\ms{valid}$ s.t. $\ms{valid} = \lit{true}$.
	Thus, all non-faulty processes (of which there are at least $n - t$) reach line \ref{line:ab:bcastecho}, broadcasting $(\ms{ID},$\ECHO$, m, \sigma)$.
	Since $n - t > \frac{n + t}{2}$, every non-faulty process will eventually receive more than $\frac{n + t}{2}$ $(\ms{ID},$\ECHO$, m, \sigma)$ messages, fulfilling the predicate at \ref{line:ab:recvechos}.
	More than $\frac{n + t}{2} > t + 1$ non-faulty processes will not have broadcast $(\ms{ID},$\READY$, m, \sigma)$, and so will do so (at line \ref{line:ab:echosbcastready}).
	Thus, all honest processes will eventually receive $t + 1$ $(\ms{ID},$\READY$, m, \sigma)$ messages, broadcasting $(\ms{ID},$\READY$, m, \sigma)$ there if not yet done.
	Then, since $n - t \geq 2t + 1$, line \ref{line:ab:twotone} will eventually be fulfilled for each non-faulty process.
Thus, every non-faulty process will ARB-deliver $(m, \sigma)$ at line \ref{line:ab:arbdeliver}, as required.}
\end{proof}

%Indeed, processes are free to propagate \READY \ messages without having received either the corresponding \INIT \ message or the \ECHO \ message from more than $\frac{n + t}{2}$ processes. Depending on the structure of the network, this flexibility may speed up convergence for non-faulty processes.

\begin{remark}
\label{arb-one-echo}
No non-faulty process will broadcast more than one message of the form $(\ms{ID},$\ECHO$, m', \sigma')$ where $\sigma'$ is such that $\sigma' = \lit{Sign}(p_x, \ms{ID}, m')$ for any message $m'$.
\end{remark}

\begin{proof}
	This follows from the proof of Lemma~\ref{arb-term-1}: if non-faulty process $p$ receives another message $(m, \sigma)$ s.t. $\sigma \leftarrow \lit{Sign}(p_x, \ms{ID}, m)$ for any $m$, then $\lit{Trace}(\ms{ID}, m, \sigma, m', \sigma') \neq$ ``indep'', and so $p$ will not reach line~\ref{line:ab:bcastecho}.
\end{proof}

\begin{lemma}
\label{arb-term-2-lemma}
In ARBP, if $p_i$ ARB-delivers $(m, \sigma)$, where $\sigma \leftarrow \lit{Sign}(p_x, \ms{ID}, m)$, and $p_j$ ARB-delivers $(m', \sigma')$, where $\sigma' \leftarrow \lit{Sign}(p_x, \ms{ID}, m')$, then $(m, \sigma) = (m', \sigma)$.
\end{lemma}
\begin{proof}
	For $p_i$ (resp. $p_j$) to have ARB-delivered $(m, \sigma)$ (resp. $(m', \sigma')$), $p_i$ (resp. $p_j$) must have broadcast $(\ms{ID},$\READY$, m, \sigma)$ (resp. $(\ms{ID},$\READY$, m', \sigma')$).
	Then, one of two predicates (at lines \ref{line:ab:recvechos} and \ref{line:ab:toneif}) must have been true for each process. That is, $p_i$ (resp. $p_j$) must have received either:
\begin{enumerate}
	\item $(\ms{ID},$\ECHO$, m, \sigma)$ (resp. $(\ms{ID},$\ECHO$, m', \sigma')$) from $\lfloor \frac{n + t}{2} \rfloor$ different processes, or
	\item $(\ms{ID},$\READY$, m, \sigma)$ (resp. $(\ms{ID},$\READY$, m', \sigma')$) from $(t + 1)$ different processes.
\end{enumerate}
We first prove the following claim: if $(\ms{ID},$\READY$, m, \sigma)$ is broadcast by $p_i$, and $(\ms{ID},$\READY$, m', \sigma')$ is broadcast by $p_j$, then $(m, \sigma) = (m', \sigma')$.
Suppose that both processes fulfill condition (1), receiving \ECHO \ messages from sets of processes $P$ and $P'$ respectively, where $p_i$ broadcasts $(\ms{ID},$\READY$, m, \sigma)$ and $p_j$ broadcasts $(\ms{ID},$\READY$, m', \sigma')$.
Assume that $(m, \sigma) \neq (m', \sigma')$. Then:
\begin{align*}
	|P \cap P'| &= |P| + |P'| - |P \cup P'|, \\
	&\geq |P| + |P'| - n, \\
	&>2\left(\frac{n + t}{2}\right) - n = t, \\
	&\Rightarrow |P \cap P'| \geq t + 1.
\end{align*}
Therefore, $P \cap P'$ must contain at least one correct process, say $p_c$. By Remark~\ref{arb-one-echo}, $p_c$ must have sent the same \ECHO \ message for some message to both processes, and so $p_i$ and $p_j$ must have received the same message $(\ms{ID},$\ECHO$, m, \sigma)$ = $(\ms{ID},$\ECHO$, m', \sigma')$, contradicting the assumption that $(m, \sigma) \neq (m', \sigma')$. Thus, they must broadcast the same \READY \ message.
% TODO - signatures may be different?
% TODO - continue from here

Suppose now that at least one process broadcasts \READY \ due to condition (2) being fulfilled.
Without loss of generality, assume exactly one process $p$ broadcasts \READY \ on this basis.
Then, $p$ must have received a \READY \ message from at least one correct process (since out of $t + 1$ processes, at least 1 must be non-faulty), say $p_a$.
Either $p_a$ received \READY \ from at least one correct process, say $p_b$, or it satisfied condition (1). By continuing the logic (and since $|P|$ is finite), there must exist a process $p_{(1)}$ that fulfilled condition (1). Then, by the correctness of processes $p_{(1)}, \dots, p_b, p_a$, \READY \ messages sent by $p_i$ and $p_j$ must be the same, completing the proof.

Therefore, $p_i$ broadcasting $(\ms{ID},$\READY$, m, \sigma)$, and $p_j$ broadcasting $(\ms{ID},$\READY$, m', \sigma')$ implies $(m, \sigma) = (m', \sigma')$ given that $p_i$ and $p_j$ are non-faulty.

We now directly prove the lemma. If $p_i$ ARB-delivers $(m, \sigma)$, it received $(\ms{ID},$\READY$, m, \sigma)$ from $(2t + 1)$ different processes, and thus received $(\ms{ID},$\READY$, m, \sigma)$ from at least one non-faulty process.
Similarly, if $p_j$ ARB-delivers $(m', \sigma')$, it must have received $(\ms{ID},$\READY$, m', \sigma')$ from at least one non-faulty process.
It follows from the previous claim that all non-faulty processes broadcast the same \READY \ message.
Thus, $p_i$ and $p_j$ ARB-deliver the same tuple.
\end{proof}

\begin{lemma}
\label{arb-term-2}
ARBP ensures ARB-Termination-2. That is, if a non-faulty process ARB-delivers $(m, \sigma)$, where $\sigma \leftarrow \lit{Sign}(\ms{ID}, p_x, m)$ was previously invoked ($p_x$ may or may not be faulty), then all the non-faulty processes eventually ARB-deliver $(m, \sigma)$.
\end{lemma}

\begin{proof}
	By Lemma \ref{arb-term-2-lemma}, all non-faulty processes that ARB-deliver a message $(m', \sigma')$ s.t. $\sigma' \leftarrow \lit{Sign}(\ms{ID}, p_x, m')$ ARB-deliver $(m, \sigma)$.
	Then, $p_i$ must have received the message $(\ms{ID},$\READY$, m, \sigma)$ from $(2t + 1)$ processes (line \ref{line:ab:twotone}), at least $t + 1$ of which must be non-faulty.
	These $t + 1$ processes must have broadcast $(\ms{ID},$\READY$, m, \sigma)$ (at line \ref{line:ab:echosbcastready} or \ref{line:ab:tone}), and so every non-faulty process will eventually receive $(t + 1)$ $(\ms{ID},$\READY$, m, \sigma)$ messages, and thus broadcast $(\ms{ID},$\READY$, m, \sigma)$ at some point.
	Given there are $n - t \geq 2t + 1$ non-faulty processes, each non-faulty process eventually receives $(\ms{ID},$\READY$, m, \sigma)$ from at least $2t + 1$ processes. Therefore, every non-faulty process will ARB-deliver $(m, \sigma)$.
\end{proof}

\begin{lemma}
\label{arb-uni}
ARBP ensures ARB-Unicity, which is stated as follows. Consider any point of time in which a non-faulty process $p$ has ARB-delivered more than one tuple. Let $delivered = \{(m_1, \sigma_1), \cdots, (m_k, \sigma_k)\}$, where $|delivered| = k$, denote the set of these tuples. For each $i \in \{1..k\}$, let $out_i = \lit{FindIndex}(\ms{ID}, m_i, \sigma_i)$ denote the output of an idealised call to $\lit{FindIndex}$. Then for all distinct pairs of tuples $\{(m_i, \sigma_j), (m_j, \sigma_j)\}$, $out_i \neq out_j$.
\end{lemma}
\begin{proof}
	We proceed by contradiction.
	Without loss of generality, suppose that $p$ ARB-delivers two tuples $(m, \sigma)$ and $(m', \sigma')$ such that $\lit{FindIndex}(\ms{ID}, m, \sigma) = \lit{FindIndex}(\ms{ID}, m', \sigma')$.
	Then, ARB-Termination-2 implies that all non-faulty processes will eventually ARB-deliver $(m, \sigma)$ and $(m', \sigma')$.
	But, Lemma \ref{arb-term-2-lemma} asserts that $\lit{FindIndex}(\ms{ID}, m, \sigma) = \lit{FindIndex}(\ms{ID}, m', \sigma')$, a contradiction.
	Thus, for each $i \in \{1..n\}$, $p$ ARB-delivers at most one tuple $(m, \sigma)$ such that $\lit{FindIndex}(\ms{ID}, m, \sigma) = i$.
\end{proof}

\begin{theorem}
\label{arb-thm}
ARBP (Algorithm~\ref{alg:arb} in Section \ref{sec:arb:arb}) satisfies the properties of ARB-Broadcast.
\end{theorem}

\begin{proof}
	From Lemmas \ref{arb-anon}, \ref{arb-val}, \ref{arb-uni}, \ref{arb-term-1} and \ref{arb-term-2}, it follows that all properties of ARB-Broadcast are satisfied.
\end{proof}

\iffalse
\begin{lemma}
TODO: remove? Given DDH and DLog problem are hard, an adversary cannot determine the value $i$ for probability $Pr > \frac{1}{n - t}$
\end{lemma}

\begin{proof}
	As the adversary can corrupt $f$ processes, they have a priori knowledge of their index, leaving $n - f$ non-faulty processes.
	Let $Pr$ denote the probability of the adversary corretly determining the index of $p$.
	We first show that $p$'s signature $\sigma$ does not increase $Pr$ given DDH is intractible.
	To this end, we construct an algorithm $\mathcal{A}$ that shows that the adversary can solve DDH with probability $\frac{1}{n - f} + \frac{\varepsilon}{2}$, which by assumption is intractible, which contradicts $Pr$ being s.t. $Pr > \frac{1}{n - f}$.
	So, suppose that the adversary has advantage $\varepsilon$ in determining $p$'s index from $\sigma$. That is, assume that $Pr = \frac{1}{n - f} + \varepsilon$.

	Consider the signature scheme proposed in \cite{Fujisaki2007}.
	Let $G$ be a multiplicative group of prime order.
	Let $inst = (g_1, g_2, u, v)$ be a given instance of the decisional DH problem, where $g_1, g_2, u, v \in G$.
	Note that when $(g_1, g_2, u, v)$ is a DDH tuple, $\log_{g_1}{u} = \log_{g_2}{v}$ holds.
	Consider the construction of $\mathcal{A}$ as described in Theorem 5.4 in  \cite{Fujisaki2007}.
	In essence, the adversary is tasked to determine the bit $b$ of the signing oracle $\lit{Sign}_{SK_b}$, given access to $\lit{Sign}_{SK_0}$, $\lit{Sign}_{SK_1}$ and $\lit{Sign}_{SK_b}$.
	We extend this construction, considering the adversary who can access $\lit{Sign}_{SK_i}$ for each $i = \{1, \cdots, n\}$, as well as $\lit{Sign}_{SK_j}$ for some hidden value $j \in \{1, \cdots, n\}$, and is tasked to determine $j$.
	Let $k$ be the adversary's chosen value in the experiment. 
	If $k = j$, then $\mathcal{A}$ returns 1, otherwise a random $r \in \{0, 1\}$.
	The probability $Correct$ of the adversary choosing $j$ corectly is computed as in \cite{Fujisaki2007} and \cite{Saberhagen2013}:
	\begin{align*}
		Guess = & \frac{1}{2} + Pr(1 \mid inst \in DDH) - PR(1 \mid inst \notin DDH) \\
		= & \frac{1}{2} + Pr(k = j \mid inst \in DDH) + Pr(k \neq j \mid inst \in DDH) Pr(r = 1) \\
		& -  Pr(k = j \mid inst \notin DDH) + Pr(k \neq j \mid inst \notin DDH) Pr(r = 0) \\
		= & \frac{1}{2} + \Big(\frac{1}{n - f} + \varepsilon\Big) + \Big(\frac{n - f - 1}{n - f} - \varepsilon\Big) \frac{1}{2} - \frac{1}{n - f} - \Big(\frac{n - f - 1}{n - f}\Big)\frac{1}{2}
	\end{align*}
	Thus, $Guess = \frac{1}{2} + \frac{\varepsilon}{2}$ as required.
\end{proof}
\fi


==> avc_state.tex <==
\begin{algorithm}[t]
\label{alg:aic-state}
\caption{AVCP: Initial state}
	% state in pseudo-code
	{\footnotesize
	\begin{algorithmic}
%		\State $config$ \Comment{Application-specific configuration proposal, initially $\perp$}
%		\State $pk, SK$ \Comment{The public/private key pair from the DKG, both initialised to $\perp$}
%		\State $\ms{BIN\_CONS}[1..n, l_1..l_n] \leftarrow \ms{BIN\_CONS}[1..n, \perp..\perp]$ \Comment{Binary consensus instance objects}
		\State $ID$  \Comment{The unique identifier for an instance of consensus}
		\State $\ms{proposals[] \leftarrow \emptyset}$ \Comment{Map with labels as keys and proposals of the form $(m, \sigma)$ as values}
		\State $\ms{bin\_decisions[] \leftarrow \emptyset}$ \Comment{Map with labels as keys and binary values as values}
		\State $\ms{labelled}[] \leftarrow \emptyset$ \Comment{Map with labels as keys and binary consensus instances as values}
		\State \ms{unlabelled} \Comment{Stack containing $n$ instances of binary consensus}
		\State $\ms{ones}[][]$ \Comment{Map of two maps with keys \EST \ and \AUX \ for each round $r$ containing labels}
		\State $\ms{counts}[][]$ \Comment{Map of two maps with keys \EST \ and AUX \ for each round $r$ containing integers, each initialised to 0}
%		\State $\ms{curr\_index} \leftarrow 1$ \Comment{The value that an instance of binary consensus will be indexed by}
%		\State $(\ms{est\_count[r]}, \ms{aux\_count[r]}) \leftarrow (\{ \}, \{ \})$ \Comment{Key-value stores where all values are initially $0$} %; uninitialised key $k$ initialises the value corresponding to $k$ to $0$}
%		\State $(\ms{est\_ones[r]}, \ms{aux\_ones[r]}) \leftarrow (\{ \}, \{ \})$  \Comment{Key-value stores where all values are initially $\emptyset$} %; querying for some uninitialised key $k$ initialises the value corresponding to $k$ to $\emptyset$}
%		\State \ms{timeout}, \ms{timer} \Comment{Timeout fixed to some common value and associated timer}
	\end{algorithmic}}
\end{algorithm}


==> avcproof/avcproof.bkp.tex <==
\section{Analysis of AVCP} \label{sec:avcproof}

In this appendix, we prove that the properties of Anonymous Proposer Vector Consensus (AVC), presented in Section~\ref{sec:avc:avc}, are satsified by our protocol Anonymous Vector Consensus Protocol (AVCP) (Algorithms \ref{alg:avc} and \ref{alg:bchandler}).
%At a high level, our proof strategy is as follows.
%Firstly, we prove that the labelling mechanism is correct (Lemma \ref{avc-labelling}), which is implicitly relied upon in the rest of our proofs.
%Then, we prove that non-faulty processes send and receive messages in a manner that preserves the properties of $n$ concurrent instances of binary consensus.
%Firstly, we consider messages of the form \MSG$[r, i](1)$  which allows us to prove that all non-faulty processes eventually decide 1 in $n - t$ instances of binary consensus (Lemma \ref{avc-reachline}), whose corresponding proposals fulfil valid() (Lemma \ref{avc-val1}), after proving a few lemmas.
%Then, we consider the propagation of zero-messages (Lemma \ref{avc-equivall}).
%Having effectively considered all components of the reduction, we proceed to prove each property of AVC individually (Theorems \ref{avc-val} to \ref{avc-anon}), completing the proof.

%We note that a process' local vector $V$ is denoted by $\ms{proposals}$ in the protocol. Further, we assume that a necessary condition for a process to be considered correct is in the ARB-broadcast of a value that satisfies valid().

\begin{lemma}
\label{avc-labelling}
In AVCP, for each identifier $\ms{ID}$, a non-faulty process' data structure ``$\ms{labelled}[]$'' is such that $|\ms{labelled}.\lit{values}| \leq n$.
Further, no two binary consensus instances are labelled by the same value $l$.

%At most $n$ binary consensus instances will be labelled, and no two labels will conflict insofar as the collision resistance of $H$ and the pre-image resistance of hash functions $H_1$ and $H_2$ invoked in the traceable ring signature scheme \cite{Fujisaki2007} holds.
\end{lemma}

\begin{proof}
	For the first part of the lemma, recall that an instance $inst$ is only moved to $\ms{labelled}$ at line~\ref{line:avc:labelinst} upon ARB-delivery of $(m, \sigma)$.
	By ARB-Unicity, a non-faulty process will ARB-deliver at most one tuple $(m, \sigma)$ for every process $p_i$ s.t. $\sigma \leftarrow \lit{Sign}(\ms{ID}, p_i, m)$.
	Since $|P| = n$, at most $n$ instances $inst$ will thus be moved to $\ms{labelled}$.

	For the second part of the lemma, recall that we assume signature uniqueness.
	Thus, every tuple $(m, \sigma)$ ARB-broadcast by a non-faulty process is unique.
	Moreover, any duplicate tuple $(m, \sigma)$, even if broadcast by a faulty process, cannot be ARB-delivered twice, by ARB-Unicity.
	Thus, by the collision-resistance of $H$, $H(m \mid \mid \sigma) \neq H(m' \mid \mid \sigma')$ for any two tuples $(m, \sigma)$ and $(m', \sigma')$ that are ARB-delivered.
	Since each instance is labelled by $H(m \mid \mid \sigma')$ for some tuple $(m, \sigma)$, it follows that no two instances will conflict in label.
%	For the first part of the Lemma, recall that an instance of \ms{BIN\_CONS} is only labelled at line \ref{line:bchandler:label}, upon the ARB-delivery of a message $m$. By ARB-Unicity, at most one message is ARB-delivered per process, and so at most $n$ instances will be labelled.

%	For the second part, suppose that two messages $m$ and $m'$ are ARB-delivered by some non-faulty process. Recall that a message that is ARB-delivered is of the form $(v, s(v))$, where $s(v)$ is the traceable ring signature of $v$ that does not trace to any other ring signatures that can be ARB-delivered (this follows from ARB-Anonymity). Recall in signature generation that a value $A_1 = i^{-1}(\sigma_i - A_0)$ comprises any valid signature, where $A_0 = H_2(L,v)$ and $\sigma_i = x_iH_1(L)$, where $x_i$ is the signer's public key. By the pre-image resistance of $H_1$, it is infeasible for an adversary to generate a particular value of $\sigma_i$ deterministically\footnote{We note that, even if an adversary could vary $L$, it is infeasible for them to generate a particular value $H_1(L)^{-1}$, since $L$ depends on $x_i$.}. Similarly, by the pre-image resistance of $H_2$, it is infeasible for an adversary to vary $v$ to deterministically generate a desired value of $A_0$. Since the other variables in $A_1$ are effectively constants, it follows that it is infeasible for an adversary to generate a value of $A_1$ that is identical to that of another ARB-deliverable signature. Since a signature comprises partially of $A_1$, and an ARB-deliverable message contains a signature, it follows that messages $m$ and $m'$ will be different overall. Given the collision-resistance of $H$, it follows that $H(m) \neq H(m')$, and since $H(m)$ labels an instance corresponding to $m$, it follows that no two labelled instances will conflict in label.
\end{proof}
% defer part about A_1 to TRS section and refer to?

\begin{lemma}
\label{avc-sameinfo}
Consider AVCP. Let $p$ be a non-faulty process. Then, given that the for loop on lines \ref{line:avc:forlooptemp2} and \ref{line:avc:delivertemp2} is executed as an atomic operation, all instances in $\ms{unlabelled}.\lit{values}()$ will contain the same set of messages.
\end{lemma}

\begin{proof}
	At the protocol's outset, all instances of binary consensus are in $\ms{labelled}$, where no messages have been received.
	The only place that messages are deposited to unlabelled instances is at lines \ref{line:avc:forlooptemp2} and \ref{line:avc:delivertemp2}, where messages are deposited into \textit{all} members of $\ms{unlabelled}$.
	Finally, note that instances can only moved out of $\ms{unlabelled}$, which occurs at line~\ref{line:avc:labelinst}.
%	Denote the set of instances labelled with $\perp$ by $L$.
%	At the protocol's outset, no values are receipt in any instance in $L$, and $|L| = n$.
%	Then, an instance $\ms{BIN\_CONS}[i, \perp]$ is potentially populated only in the block beginning at line \ref{line:bchandler:receiptzeros} upon receipt of a message of the form $($\MSG$, 0, r, \neg S=\{l_1, \cdots, l_k\})$.
%	For such a message to be processed, labels must eventually be assigned to instances of the form $\ms{BIN\_CONS}[i, label]$ s.t. $label \in S$ for all $label \in S$ (line \ref{line:bchandler:label}).
%	Given this holds, the same message \MSG$[r, \perp](0)$ is deposited into all instances in $L$ (line \ref{line:bchandler:zeroperpdep}), the only time where $L$ is populated.
%	This holds for the lifetime of the protocol as $L$ only shrinks in size from the protocol's outset.
\end{proof}

\begin{lemma}
\label{avc-labelsend}
In AVCP, a non-faulty process $p$ sends a message of the form $(\ms{ID}, $\TAG$, r, \ms{label}, b)$, then there locally exists an instance of binary consensus $inst$ such that $\ms{labelled}[\ms{label}] = inst$.
\end{lemma}

\begin{proof}
Suppose $p$ sends $(\ms{ID}, $\EST$, r, \ms{label}, b)$.
If $b = 1$, then one of three scenarios holds:
\textit{(i)} $r = 1$ and $p$ has invoked $inst.\lit{bin\_propose}(1)$ where $\ms{labelled}[\ms{label}] = inst$,
\textit{(ii)} $r \geq 1$, $p$ has received $t + 1$ messages of the form  $(\ms{ID}, $\EST$, r, \ms{label}, b)$ and has not yet broadcast $(\ms{ID}, $\EST$, r, \ms{label}, b)$, or
\textit{(iii)} their value $est$ was set to $b = 1$ at the end of the previous round of binary consensus.
In case (i), note that $\lit{bin\_propose}(1)$ (at line~\ref{line:avc:invokebpone}) is executed after $inst$ is labelled (at line~\ref{line:avc:labelinst}).
Note that in both cases (ii) and (iii), $p$ must have processed messages of the form $(\ms{ID}, $\EST$, r, \ms{label}, 1)$.
As described in the text, these messages are only processed \textit{after} the ARB-delivery of the corresponding message $(m, \sigma)$ where $\ms{label} = H(m \mid \mid \sigma)$ and some instance $inst$ is labelled by $\ms{label}$ (at line~\ref{line:avc:labelinst}).
If $b = 0$, only case (ii) needs to be considered, since the other $\lit{broadcast}$ call is handled by the handler (Algorithm~\ref{alg:bchandler}).
Here, $b = 1$ must have been initially broadcast, which is described by cases (i) and (iii).
Suppose $p$ sends $(\ms{ID}, $\AUX$, r, \ms{label}, b)$.
Note that $b \neq 0$, since the handler handles this case. %TODO: elaborate slightly
Thus, we consider $b = 1$.
$b$ must have been BV-delivered (line \ref{line:obc:bvalsnonempty} of Algorithm~\ref{alg:obc}), requiring $p$ to have processed messages of the form $(\ms{ID}, $\EST$, r, \ms{label}, b)$, which requires some instance to be labelled by $\ms{label}$ to do.
This exhausts the possibilities.
\end{proof}

\begin{lemma}
\label{avc-deposit}
%Suppose a non-faulty process ARB-broadcasts $m$. Then, all messages sent by any non-faulty process relating to $m$ will eventually be deposited into some instance $\ms{BIN\_CONS}[i, H(m)]$ by all non-faulty processes.
Consider AVCP. Let $r \geq 1$ be an integer. Then, all messages sent by non-faulty processes of the form $(\ms{ID}, $\TAG$, r, \ms{label}, b)$ where \TAG \ $\in$ $\{$\EST $,$ \AUX $\}$ and $b \in \{0, 1\}$, and $(\ms{ID}, $\TAG$, r, ones)$ where \TAG \ $\in$ $\{$\ESTONES $,$ \AUXONES $\}$ and $b \in \{0, 1\}$, are eventually deposited into the corresponding binary consensus instances of a non-faulty process.
\end{lemma}

\begin{proof}
	Let $p$ be the recipient of a message in the above forms.
	We first consider messages of the form $(\ms{ID}, $\TAG$, r, \ms{label}, b)$ where \TAG \ $\in$ $\{$\EST $,$ \AUX $\}$ and $b \in \{0, 1\}$.
	By Lemma~\ref{avc-labelsend}, the non-faulty sender of such a message must have ARB-delivered some message $(m, \sigma)$ such that $\ms{label} = H(m \mid \mid \sigma)$.
	By ARB-Termination-2, $p$ will eventually ARB-deliver $(m, \sigma)$ and subsequently label an instance of binary consensus which uniquely defined by $\ms{label}$ (Lemma~\ref{avc-labelling}).
	Thus, $p$ will eventually process $(\ms{ID}, $\TAG$, r, \ms{label}, b)$ in instance $inst = \ms{labelled}[\ms{label}]$.
	Consider messages of the form $(\ms{ID}, $\TAG$, r, ones)$ where \TAG \ $\in$ $\{$\ESTONES $,$ \AUXONES $\}$ and $b \in \{0, 1\}$.
	Since the sender is non-faulty, every element of $ones$ (i.e. every label) must correspond to a message that was ARB-delivered by the sender.
	By ARB-Termination-2, $p$ will eventually ARB-deliver these messages, label instances of binary consensus (at line \ref{line:avc:labelinst}) and thus progress beyond line~\ref{line:avc:wuntillabel}.
	Thus, $p$ will deposit 0 in all instances \textit{not} labelled by elements of $ones$ (at lines \ref{line:avc:delivertemp1} and \ref{line:avc:delivertemp2}), which is the prescribed behaviour.
\end{proof}

%	We first note that, by ARB-Termination-1, all non-faulty processes will ARB-deliver $m$, and as such will label some instance $\ms{BIN\_CONS}[i, H(m)]$ (at line \ref{line:bchandler:label}). We will implicitly use this fact throughout the proof.

%	Let $p$ be a non-faulty process. Then, there are three types of messages that non-faulty processes can send, noting that \MSG \ $\in\{$\EST$, $\AUX$\}$:
%\begin{enumerate}
%	\item Messages of the form $($\MSG$, 0, r, \neg S=\{l_1, \cdots, l_k\})$
%	\item Messages of the form \MSG$[r, label](1)$
%	\item Messages of the form \EST$[r, label](0)$
%\end{enumerate}

%Let $M_1$ denote the set of messages (sent by non-faulty processes) received by $p$ of form 1, and $M_{2, 3}$ denote the set of messages sent by non-faulty processes of form 2 or 3.

%Consider $M_1$. Let $A$ be the set of messages in $M_1$ where $m \in S$, and $B$ be the messages in $M_1$ where $m \notin S$. For messages in $B$ that reach line \ref{line:bchandler:zerodep} prior to $m$'s ARB-delivery, by Lemma \ref{avc-sameinfo}, the (zero) messages corresponding to $m$ (and all other values in $S^c \cup \perp$) will be deposited in all instances of the form $\ms{BIN\_CONS}[i, \perp]$. For messages in $B$ that reach line \ref{line:bchandler:zerodep} after ARB-delivery of $m$, the message will be deposited in some $\ms{BIN\_CONS}[i, label]$, where $label \leftarrow H(m)$ prior at line \ref{line:bchandler:label}, since $H(m) \in S^{c}$. Then, considering $A$: since $x \in S$ for all messages in $A$, $x \notin (S^{c} \cup \perp)$ for all messages in $A$, and so messages are not deposited at lines \ref{line:bchandler:zerodep} or \ref{line:bchandler:zeroperpdep}, as expected.

%Consider $M_{2, 3}$. Prior to ARB-delivery of a message $m$, all messages in $M_{2,3}$ such that $label = H(m)$ are buffered by $p$ (at line \ref{line:bchandler:bufferones}) until ARB-delivery of $m$ when they are deposited into an instance.
%\end{proof}

%Messages being deposited into instances does not imply that they are handled as in a normal instantiation of $\ms{BIN\_CONS}$ (c.f. Appendix \ref{sec:bvbincons}), and so we show this for messages of the form \MSG$[r, label](b)$, where \MSG $\in \{$\EST$, $\AUX$\}$ and $b = 1$, and later show this holds, given that all instances make progress, for any $b \in \{0, 1\}$ also.

%\begin{lemma}
%\label{avc-equivones}
%Let $t < \frac{n}{3}$. For some non-faulty process $p$, invoking AVC\_BV\_broadcast \EST$[r,H(m)](1)$ or broadcast \AUX$[r,H(m)](1)$ is equivalent to broadcasting \EST$[r,H(m)](1)$ or \AUX$[r,H(m)](1)$ respectively.
%\end{lemma}

%\begin{proof}
%	Let $p$ be a non-faulty process. Consider round $r = 1$. To propose 1 in some instance $\ms{BIN\_CONS}$, $p$ must have ARB-delivered a valid message $m$ (lines \ref{line:avc:ifvalid} and \ref{line:avc:binpropone}), and thus must have labelled an instance $\ms{BIN\_CONS}[i, H(m)]$. Then, adding $H(m)$ to $\ms{est\_ones}[1]$ is clearly possible (at line \ref{line:bchandler:popestones}). Then, $p$ BV-broadcasts \EST$[r,H(m)](1)$. By ARB-Termination-2, all non-faulty processes will eventually ARB-deliver $m$, and by Lemma \ref{avc-deposit} they will eventually process $p$'s message in $\ms{BIN\_CONS}[H(m)]$.

%	Then, suppose that in some instance $\ms{BIN\_CONS}[i, H(m)]$, $p$ begins some round $r > 1$ with $est_{H(m)} = 1$. By BV-Justification and construction of the binary consensus routine, $est_{H(m)}$ must have been proposed in round $r - 1$ by at least one non-faulty process. As such, if not yet ARB-delivered, by the correctness of that process and ARB-Termination-2, $p$ will eventually ARB-deliver $m$, and will thus be able to invoke BV-broadcast in line \ref{line:bchandler:bvone}. By the same reasoning applied in the case of $r = 1$, it follows that all proposals of the form \EST$[r, H(m)](1)$ will be suitably broadcast and received by all non-faulty processes.

%	The proof for messages of the form \AUX$[r, H(m)](1)$ is similar. For a process to propose \AUX$[r,H(m)](1)$, $\ms{bin\_values_{H(m)}}$ must have been populated with 1 (line \ref{line:bincons:bvalsnonempty}). By BV-Justification, 1 must have been proposed by a non-faulty process. Such a process must have ARB-delivered $m$ in order to propagate such a message. Since $p$ will eventually ARB-deliver $m$ (ARB-Termination-2), $p$ is able to label an instance $\ms{BIN\_CONS}[i, H(m)]$ for some $i$, and can as such broadcast \AUX$[r,H(m)](1)$.
%\end{proof}

%\begin{lemma}
%	\label{avc-bvbroadcast}
%	Let $t < \frac{n}{3}$. A non-faulty process can propagate a message of the form \EST$[r,label](b)$ upon its receipt from $t + 1$ processes (as in line \ref{line:bincons:tplusone}), where $b \in \{0, 1\}$. Moreover, the properties of BV-broadcast are preserved.
%\end{lemma}

%\begin{proof}
%	Suppose a non-faulty process $p$ invokes BV-broadcast with \EST$[r,label](b)$, where $b = 1$. This requires $p$ to have previously labelled some instance $\ms{BIN\_CONS}[i,label]$ (at line \ref{line:bchandler:bvbroadcastlabel}). Therefore, $p$ must have ARB-delivered some $v$ s.t. $H(v) = label$. Then, suppose $p$ receives \EST$[r, label](0)$ messages from $t + 1$ processes. Then, $p$ will not block at line \ref{line:bincons:notlabelled}, and will broadcast \EST$[r, label](0)$. Suppose then $b = 0$. Then, suppose $p$ receives \EST$[r, label](1)$ from $t + 1$ processes. Then, at least one non-faulty process must have sent \EST$[r, label](1)$, who must have labelled an instance of binary consensus $\ms{BIN\_CONS}[i, label]$ for some $i$, and therefore must have ARB-delivered the corresponding value $v$ s.t. $H(v) = label$. Then, by ARB-Termination-2, $p$ will eventually ARB-deliver $v$, label an instance $\ms{BIN\_CONS}[i, label]$, therefore fulfilling line \ref{line:bincons:notlabelled}, and broadcast \EST$[r, label](1)$ as required. We note that if $p$ invokes \EST$[r,label](b)$, and then receives \EST$[r, label](b)$ from $t + 1$ processes, $p$ does not broadcast again (i.e. does not fulfil the conditions at line \ref{line:bincons:tplusone}).

%\end{proof}

\begin{lemma}
	\label{avc-reachline}
	In AVCP, every non-faulty process reaches line \ref{line:avc:binpropzeros}, i.e. decides 1 in $n - t$ instances of binary consensus.
\end{lemma}

\begin{proof}
	Given at most $t$ faulty processes, at least $n - t$ non-faulty processes invoke ARB-broadcast at line \ref{line:avc:arbbcast}, broadcasting a value that satisfies $\lit{valid}()$ by assumption.
	By ARB-Termination-1, every message ARB-broadcast by a non-faulty process is eventually ARB-delivered by all non-faulty processes.
	Suppose a non-faulty process $p$ labels an instance of consensus $\ms{inst}$ by one of these messages.
	By Lemma~\ref{avc-deposit}, all messages sent by non-faulty processes associated with $\ms{inst}$ are eventually processed by $p$.
	Then, all non-faulty processes will invoke $\lit{bin\_propose}(1)$ in at least $n - t$ instances of binary consensus (i.e. while blocked at line~\ref{line:avc:wuntilnminust}).
	Consider the first $n - t$ instances of consensus for which a decision is made at.
	By the intrusion tolerance of binary consensus, no coalition of faulty processes can force 0 to be a valid value in these consensus instances, since all non-faulty processes must invoke $\lit{bin\_propose}(1)$ in them. %TODO: reword %TODO: reword %TODO: reword %TODO: reword
	Then, by BBC-Agreement, BBC-Validity and BBC-Termination, all non-faulty processes will eventually decide 1 in $n - t$ $\ms{BIN\_CONS}$ instances.
	Thus, all non-faulty processes eventually reach line \ref{line:avc:binpropzeros}.
\end{proof}

We now prove that AVC-Validity holds.

\begin{theorem}
\label{avc-val}
AVCP satisfies AVC-Validity, which is stated as follows. Suppose a process $p$ proposes the value $v$. Then, if $v$ is decided by some non-faulty process, then it must satisfy $\lit{valid}()$. Further, at least $n - t$ values that satisfy $\lit{valid}()$ must eventually arrive in a non-faulty process's vector $V$.

\end{theorem}

\begin{proof}
	Let $p$ be a non-faulty process.
	By construction of the binary consensus algorithm, $p$ must process messages of the form $(\ms{ID}, $\TAG$, r, \ms{label}, b)$ where \TAG \ $\in$ $\{$\EST $,$ \AUX $\}$ and $b \in \{0, 1\}$ to reach a decision.
	By Lemma~\ref{avc-deposit}, $p$ must have ARB-delivered the corresponding message $(m, \sigma)$ such that $\ms{label} = H(m \mid \mid \sigma)$ before deciding.
	That is, $\ms{proposals}$ must have been populated with the corresponding message $(m, \sigma)$ at line~\ref{line:avc:addtoprops}, and $\lit{valid}()$ must be true for $(m, \sigma)$, checked previously at line~\ref{line:avc:ifvalid}.
	By Lemma \ref{avc-reachline}, $p$ eventually decides 1 in $n - t$ instances of binary consensus.
	Upon each decision, the corresponding message is added to $V = \ms{decided\_ones}$ (at line~\ref{line:avc:addone}).
\end{proof}

% all unlabelled are identical, so will terminate at same time
\begin{lemma}
\label{avc-equivall}
%Let $t < \frac{n}{3}$. Then, fixing $r$, if AVC\_BV\_broadcast \EST$[r,label](b_{label})$ or broadcast \AUX$[r,label](b_{label})$ is invoked in all $n$ instances of $\ms{BIN\_CONS}$ by a non-faulty process, then all non-faulty processes eventually process \EST$[r,label](b_{label})$ or \AUX$[r,label](b_{label})$ (respectively) in all $n$ instances.
Consider AVCP. Fix $r \geq 1$. If a non-faulty process $p$ invokes ``$\lit{broadcast}$ $(\ms{ID}, $\EST$, r, \ms{label}, b)$'' or ``$\lit{broadcast}$ $(\ms{ID}, $\AUX$, r, \ms{label}, b)$'' in all $n$ instances of binary consensus, then all non-faulty processes interpret the corresponding messages sent by $p$ as if $p$ were executing the original binary consensus algorithm.
\end{lemma}

\begin{proof}
	Without loss of generality, suppose $p$ invokes ``$\lit{broadcast}$ $(\ms{ID}, $\EST$, r, \ms{label}, b)$'' in all $n$ instances of binary consensus.
	For every instance $inst$ such that $b = 1$, $p$ broadcasts $(\ms{ID}, $\EST$, r, \ms{label}, b)$ (at line~\ref{line:avc:bcastest}) which is identical to the behaviour in the original algorithm.
	Note that $p$ does not broadcast $(\ms{ID}, $\EST$, r, \ms{label}, b)$ here when $b = 0$.
	By Lemma~\ref{avc-labelsend}, $p$ must have labelled $inst$ with $\ms{label}$. Thus, $p$ adds $\ms{label}$ to $\ms{ones}[$\EST$][r]$ (at line \ref{line:avc:appendonesest}).
	Once $n$ invocations of ``$\lit{broadcast}$ $(\ms{ID}, $\EST$, r, \ms{label}, b)$'' have been executed, $\ms{ones}[$\EST$][r]$ is sent to all non-faulty processes.
	By Lemma~\ref{avc-deposit}, all non-faulty processes deposit $0$ in all instances not labelled by elements of $\ms{ones}[$\EST$][r]$, corresponding to all broadcasts \textit{not} performed by $p$ previously.
	In this sense, this behaviour is equivalent to having broadcast all values $(\ms{ID}, $\EST$, r, \ms{label}, b)$ where $b = 0$.
%	Consider an arbitrary round $r$.
	
%	Firstly, consider messages of the form \EST$[r,label](b_{label})$. By Lemma \ref{avc-equivones}, all messages of the form \EST$[r,label](1)$ are handled. So, we consider messages of the form \EST$[r,label](0)$. To propose 0 in some instance $\ms{BIN\_CONS}$, $p$ must have incremented $est\_count[r]$ to $n$ (on reaching line \ref{line:bchandler:incestcount} $n$ times, having stored all proposed 1's in $\ms{est\_ones}[r]$ at line \ref{line:bchandler:popestones} prior). Then, $p$ broadcasts $($\EST$, 0, r, \neg \ms{est\_ones}[r])$, corresponding to proposing zeroes in all other instances not labelled by elements in $\ms{est\_ones}[r]$. Then, at line \ref{line:bchandler:waitzeroarb}, by $p$'s correctness and ARB-Termination-2, all values in $\ms{est\_ones}[r]$ will be eventually known by all non-faulty processes, and so will consider \EST$[r,i](0)$ as receipt for all $i \notin \ms{est\_ones}[r]$. Moreover, every round will be considered, as $p$ does not terminate upon deciding.

%	Now, consider messages of the form \AUX$[r,label](b_{label})$. By Lemma \ref{avc-equivones}, all proposals of 1 are handled. Then, let $p$ denote a non-faulty process. Consider the proposal of \AUX$[r,H(m)](0)$. By the same reasoning as above, $p$ will eventually reach line \ref{line:bchandler:bcastauxzeros}, broadcasting $($\AUX$, 0, r ,\neg \ms{aux\_ones[r]})$, and since $p$ is non-faulty, all other non-faulty processes will eventually reach line \ref{line:bchandler:zerodep}, depositing all zero values into relevant instances of $\ms{BIN\_CONS}$.
\end{proof}

%Aside: Suppose that a process $p$ decides in round $r$ in some instance of binary consensus. Then, after round $r + 2$, in the associated terminating binary consensus algorithm of \cite{Crain2017a}, $p$ can halt while preserving the liveness and safety of all non-faulty processes. Thus, over all instances of $\ms{BIN\_CONS}$, $p$ can halt after round $r_{max} + 2$, where $r_{max}$ is the largest value of $r$ for which $p$ decides in, thus preserving liveness and safety guarantees in all instances.

%Having proven relevant properties about the binary consensus handler, we proceed to prove properties of $AVC$ are fulfilled by the algorithm $anon-vc$. To do so, we assume BBC-Validity, BBC-Agreement and BBC-Termination holds in any standalone instance of binary consensus. % fair?

%\begin{lemma}
%\label{avc-val2}
%For every non-faulty process that decides, if $v \in V$, then $v$ must satisfy $\lit{valid}()$. 
%\end{lemma}

%\begin{proof}
%	If $v = (m, \sigma)$ is ARB-broadcast by a non-faulty process, then, at some point in time, there are three possible scenarios that any other non-faulty process $p$ may be in.
%	Suppose $(m, \sigma)$ satisfies valid().
%	Then, if $(m, \sigma)$ is ARB-delivered before the process reaches line \ref{line:avc:binpropzeros}, $\ms{BIN\_CONS}[i, H(v)]$.bin\_propose(1) will be invoked. Otherwise, a process will propose 0 in all other \ms{BIN\_CONS} instances, one of which corresponds to $v$. Since $p$ has therefore proposed in all $\ms{BIN\_CONS}$ instances, by Lemmas \ref{avc-equivall} and \ref{avc-bvbroadcast}, progress in each $\ms{BIN\_CONS}$ instance is made as if they were all labelled instances. Then, by BBC-Validity, BBC-Agreement and BBC-Termination, the instance of \ms{BIN\_CONS} will eventually terminate with some $b \in \{0, 1\}$ for all non-faulty processes, where $v$ will be deposited into $V$ iff $b = 1$. Finally, if $v$ does not satisfy valid(), then no non-faulty process will invoke $\ms{BIN\_CONS}[i, H(v)]$.bin\_propose(1), and so by the intrusion-tolerance of the binary consensus routine, no non-faulty process will decide $v$.
%\end{proof}

%\begin{theorem}
%\label{avc-val}
%AVCP ensures AVC-Validity, which is stated as follows. Consider each non-faulty process that decides. Then, suppose a process $p_i$ proposes the value $v$. Then, if $v$ is decided by some non-faulty process, then it must satisfy valid(). Further, at least $n - t$ values that satisfy valid() must eventually arrive in a non-faulty process's vector $V$.
%\end{theorem}

%\begin{proof}
%The combination of Lemmas \ref{avc-val1} and \ref{avc-val2}, which characterise AVC-Validity, are proven above.
%\end{proof}

\begin{theorem}
\label{avc-term}
AVCP ensures AVC-Termination. That is, every non-faulty process eventually decides on a vector of proposals.
\end{theorem}

\begin{proof}
	Consider a non-faulty process $p$.
	By Lemma \ref{avc-reachline}, $p$ reaches line \ref{line:avc:binpropzeros} with $n - t$ values in their local array $\ms{decided\_ones}$.
	At this point, $p$ invokes $\lit{bin\_propose}(0)$ in all other instances of binary consensus.
	Since all $n$ instances are thus executed, $p$ will eventually invoke ``$\lit{broadcast}$ $(\ms{ID}, $\EST$, r, \ms{label}, b)$'' in all $n$ instances of binary consensus.
	By Lemma~\ref{avc-equivall}, non-faulty processes interpret $p$'s corresponding messages as if $p$ were executing the original binary consensus algorithm.
	Similarly, $p$ will eventually invoke ``$\lit{broadcast}$ $(\ms{ID}, $\AUX$, r, \ms{label}, b)$'' in all $n$ instances.
	Moreover, the termination condition described in the text is such that processes only halt in round $r_{max} + 2$, where $r_{max}$ is the largest round value for which $p$ decided in an instance of binary consensus.
	Thus, by BBC-Termination, every instance will eventually terminate with a decided value.
	At this point, $p$ immediately returns $\ms{decided\_ones}$ (at line \ref{line:avc:returnprops}).
	Since $p$ was arbitrary (but non-faulty), it follows that AVC-Termination holds.
\end{proof}

\begin{theorem}
\label{avc-agree}
AVCP ensures AVC-Agreement. That is, all non-faulty processes agree on the same vector of proposals $V = \{v_1, \dots\}$.
\end{theorem}

\begin{proof}
	Consider two non-faulty processes, $p_i$ and $p_j$ that have decided (AVC-Termination).
	Suppose that $p_i$ has decided $\ms{decided\_ones}$.
	Each value in $\ms{decided\_ones}$ must have been ARB-delivered to $p_i$ in order to decide 1 in the corresponding instances of binary consensus (Lemma~\ref{avc-labelsend}). % at line x?
	By ARB-Unicity and ARB-Termination-2, $p_j$ will ARB-deliver all values in $\ms{decided\_ones}$.
	By Lemma~\ref{avc-reachline}, all non-faulty processes eventually decide 1 in $n - t$ instances of binary consensus.
	Consequently, $p_i$ and $p_j$ participate in all $n$ instances of binary consensus which by Lemma~\ref{avc-equivall} is equivalent to participating in $n$ instances of binary consensus as per the original algorithm.
	Then, by BBC-Agreement, $p_j$ decides 1 in an instance of binary consensus if and only if $p_i$ decides 1 in that instance.
	Consequently, each corresponding value, which have all been ARB-delivered prior to deciding 1 in each instance of binary consensus (Lemma~\ref{avc-labelsend}) will be added to $p_j$'s local array $\ms{decided\_ones}'$.
	Thus, $\ms{decided\_ones}' = \ms{decided\_ones}$.

%	By Lemma \ref{avc-reachline}, at least $n - t$ 1's are decided, and the corresponding proposals are deposited in $p_i$ and $p_j$'s $\ms{decided\_ones}$ arrays.
%	Consider a particular instance $inst$ that decides 1 at this point.
%	By the intrusion tolerance of the binary consensus routine, a non-faulty process must have invoked $inst.\lit{bin\_propose}(1)$.
%	Since this can only be issued at line \ref{line:avc:invokebpone}, after the ARB-delivery of $(m, \sigma)$, it follows from ARB-Unicity and ARB-Termination-2 that all non-faulty processes ARB-deliver $(m, \sigma)$
%	In particular, given $p_i$ labels an instance $H(m \mid \mid \sigma)$, $p_j$ eventually will too.
%	Moreover, by Lemma \ref{avc-deposit}, all messages sent by non-faulty processes relating to \ms{inst} will eventually be processed by $p_i$ and $p_j$.
%	Then, by BBC-Agreement, for all instances of binary consensus for which $p_i$ decides 1 in, so too does $p_j$.
%	Then, all labels of instances for which 1 is decided in are added to the respective set $\ms{decided\_ones}$.
%	By AVC-Termination, $p_i$ and $p_j$ eventually return $\ms{decided\_ones}_i = \ms{decided\_ones}_j$.
%	Since $p_i$ and $p_j$ were arbitrary non-faulty processes, it it follows that AVC-Agreement holds.
\end{proof}
We restate the definition of AVC-Anonymity, then prove it holds under arbitrary composition in a restricted setting and sequential composition in a general setting under different assumptions:
	Let $msg = (m, \sigma)$ be the value proposed by a non-faulty process $p_i$.
	Then, it is impossible for the adversary to determine the value of $i$ with probability $Pr > \frac{1}{n - t}$.

\begin{theorem}
\label{avc-anon}
AVCP ensures AVC-Anonymity under arbitrary composition under the assumptions of our model (Section~\ref{sec:model:model}) and the following independence assumption.
For every instance of AVCP, the identifier $ID$ and all values proposed by non-faulty processes must not be derived from other instances of consensus.
\end{theorem}

\begin{proof}
	The proof for this claim follows similarly from the proof of AVC-Anonymity (Lemma~\ref{arb-anon}).
	The strategy is to assert the following.
	By properties of the signature scheme and independence of messages between instances, the adversary cannot determine if a a non-faulty process has anonymously broadcast their proposal or not based on whether or not they have made $\lit{send}$ calls.
\end{proof}

It is important to identify that our assumptions consider an adversary who attempts to deterministically de-anonymise a given non-faulty process.
Considering the above assumptions, suppose that $n - 1$ processes are located in a data centre, and one (non-faulty) process $p$ is located far away from those processes.
Suppose that all processes ARB-broadcast a message.
Then, based on observing the relatively late arrival of a single anonymous proposal, the adversary may \textit{correlate} $p$'s proposal with this timing information.
Under our assumptions, however, the adversary cannot determine with certainty that the late message is $p$'s.
For example, one of the $n - t - 1$ remaining non-faulty processes may be slow, and $p$ may have executed $\lit{anon\_broadcast}$ before the other $n - t - 2$ non-faulty processes.
In practice, this may not be sufficient, and so we remark that important future work is to establish a more practical model for anonymity that provides some guarantees with respect to timing information.

\begin{theorem}
\label{avc-anon2}
AVCP ensures AVC-Anonymity under arbitrary composition under the assumptions of our model (Section~\ref{sec:model:model}) and the following two assumptions:
\textit{(i)} There exists a sufficiently large window of synchrony, which starts after all non-faulty processes have decided in the previous instance of AVCP (if it exists) at the beginning of any execution of AVCP in which all non-faulty processes ARB-broadcast their proposal, and
\textit{(ii)} Non-faulty processes do not participate in a given instance of AVCP apart from anonymously broadcasting their signed proposal (at line~\ref{line:ab:initbcast} of Algorithm~\ref{alg:arb}) until the window of synchrony has elapsed.
\end{theorem}

\begin{proof}
	Without loss of generality, we consider a scenario where a new instance of AVCP has been initiated while another is executing.
	As in the case of Theorem~\ref{avc-anon2} and Lemma~\ref{arb-anon}, the adversary can only determine the signer of messages produced by corrupted processes, of which there are up to $t$.
	By assumption, all non-faulty processes ARB-broadcast their proposal in a period of synchrony.
	Notably, non-faulty processes do not propagate messages relating to the previous instance of AVCP nor in the current instace of AVCP.
	Consequently, the adversary does not learn any additional information about any non-faulty process' proposals.
	Consider a non-faulty process $p$.
	Since the network is asynchronous after the synchrony window, the adversary cannot profile $p$ based on their speed while subsequently participating in AVCP.
\end{proof}


==> bincons.tex <==
\begin{algorithm}[t]
	% state in pseudo-code
	\caption{AVCP: Binary consensus}
	{\footnotesize
	\label{alg:bincons}
	\begin{algorithmic}[1]
		\algrestore{alg:avc}
		\Part{$\lit{bin-cons}(v_{label}, label)$} {
		\State $\ms{est_{label} \leftarrow v_{label}}$; $r_{label} \leftarrow 0$;
		\Repeat
		\State $r_{label} \leftarrow r_{label} + 1$;
		\State $\lit{AVC\_BV\_broadcast}[r_{label}, label](\ms{est_{label}})$ \label{line:bincons:avcbvbcast}
		\WUntil $(\ms{bin\_values_{label}} \neq \emptyset)$ \label{line:bincons:bvalsnonempty} \EndWUntil
		\State $\lit{AVC\_AUX\_broadcast}[r_{label}, label](\ms{bin\_values_{label}})$ \label{line:bincons:avcauxbcast}
		\WUntil messages {\scriptsize $\lit{AUX}$}$[r_{label}, label](\ms{b\_val_p}(1))$, $\cdots$, {\scriptsize $\lit{AUX}$}$[r_{label}, label](\ms{b\_val_p}(n - t))$ have 
		\Statex \T\T\T been received from $(n - t)$ processes $p(x), 1 \leq x \leq n - t$ with contents s.t. 
		\Statex \T\T\T $\exists$ $values_{label} \neq \emptyset$ where the following two conditions hold:
		\T\begin{itemize}[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt,itemindent=0em,listparindent=1em,leftmargin=5em]

		\item $values_{label} = \cup_{1 \leq x \leq n - t}\ms{b\_val_{p(x)}}$
		\item $values_{label} \subseteq \ms{bin\_values_{label}[r, label]}$
		\end{itemize} \EndWUntil
		\State $b \leftarrow r_{label} \pmod{2}$
		\If{$values_{label} = \{v\}$}
		\State $est_{label} \leftarrow v$;
		\If{$v = b$}
		$\lit{decide}(v)$ if not yet invoked $\lit{decide}()$
		\EndIf
		\Else{} 
		$est_{label} \leftarrow b$
		\EndIf
		\EndRepeat
		}\EndPart
		\Statex
		\Part{$\lit{BV-broadcast}$({\scriptsize $\lit{MSG}$}$[r_{label}, label](v_i)$)} {
			\State $\lit{broadcast}$ {\scriptsize $\lit{B\_VAL}$}$[r_{label}, label](v_i)$ \label{line:bincons:initialbcast}
		}\EndPart
		\Upon{receipt of {\scriptsize $\lit{B\_VAL}$}$[r_{label}, label](v)$}
		\If{{\scriptsize $\lit{B\_VAL}$}$[r_{label}, label](v)$ received from $(t + 1)$ processes and 
		\Statex\T\T {\scriptsize $\lit{B\_VAL}$}$[r_{label}, label](v)$ not yet broadcast} \label{line:bincons:tplusone}
		\If{$\ms{BIN\_CONS}$ not labelled} \WUntil $label$ labels $\ms{BIN\_CONS}$ \EndWUntil \EndIf \label{line:bincons:notlabelled}
		\State $\lit{broadcast}$ {\scriptsize $\lit{B\_VAL}$}$[r_{label}, label](v)$ \label{line:bincons:nowlabelled}
		\EndIf
		\If{{\scriptsize $\lit{B\_VAL}$}$[r_{label}, label](v)$ received from $(2t + 1)$ processes} \label{line:bincons:twotplusone}
		\State $\ms{bin\_values_{label}} \leftarrow \ms{bin\_values_{label}} \cup \{v\}$
		\EndIf
		\EndUpon
	\algstore{alg:bincons}
	\end{algorithmic}
	}
\end{algorithm}


==> decryptbals.tex <==
\begin{algorithm}[htp]
\label{alg:decryptbals}
{\small 
	% state in pseudo-code
	\caption{Ballot decryption}
	\begin{algorithmic}[1]
		\algrestore{alg:election}
		\Part{Initial State} {
			\State $\ms{partial-decs} \leftarrow \emptyset$ \Comment{local partial decryptions of \ms{enc-ballots}} \label{line:dec:partialdecs}
			\State $\ms{buffered-decs} \leftarrow \emptyset$ \Comment{key-value store: keys correspond to labels, values correspond to valid share decryptions} \label{line:dec:buffereddecs}
		\State $\ms{ballots-decs} \leftarrow \emptyset$ \Comment{set containing (decrypted) ballots} \label{line:dec:ballots}
		\State $\ms{has-broadcast} \leftarrow$ False \Comment{Boolean corresponding to whether or not partial decryptions have been boradcast} \label{line:dec:hasbcastvar}
		\Statex
		}\EndPart
		\Part{decrypt-ballots(\ms{enc-ballots})} {
		\For{each $bal$ in $\ms{enc-ballots}$} \label{line:dec:foreach}
		\State $\ms{partial-decs} \leftarrow \ms{partial-decs}$ $\cup$ $(H(bal)$, partial-decryption($bal$)$)$ \label{line:dec:partialinc}
		\EndFor
		\For{each $(label, dec)$ in $\ms{partial-decs}$} \label{line:dec:foreachownshare}
		\State $\ms{buffered-decs}[label] \leftarrow \ms{buffered-decs}[label] \cup dec$ \label{line:dec:addownshare}
		\EndFor
		\State Broadcast \ms{partial-decs} \label{line:dec:bcast}
		\State $\ms{has-broadcast} \leftarrow$ True \label{line:dec:true}
		\Statex
	}\EndPart
		\Upon{receipt of $\ms{decs}$}
		\If{valid-decs($\ms{decs}$)} \label{line:dec:validdecs}
		\WUntil \ms{has-broadcast} is True \EndWUntil
		\For{each $(label, dec)$ in $\ms{partial-decs}$}
		\State $\ms{buffered-decs}[label] \leftarrow \ms{buffered-decs}[label] \cup dec$ \label{line:dec:incbuffer}
		\EndFor
		\If{$|\ms{buffered-decs}[k]| \geq t + 1$ for all keys $k$} \label{line:dec:enoughshares}
			\For{each key $k$ of \ms{buffered-decs}} \label{line:dec:foreachbuffered}
			\State $\ms{ballots} \leftarrow \ms{ballots}$ $\cup$ combine-shares($\ms{buffered-decs}[k]$) \label{line:dec:combineshares}
			\EndFor
			\Return \ms{ballots} \EndReturn \label{line:dec:return}
			\EndIf
		\EndIf
		\EndUpon
	\end{algorithmic}}
\end{algorithm}


==> election.tex <==
\begin{algorithm}[htp]
\label{alg:election}
{\small
	% state in pseudo-code
	\caption{Arbitrary ballot election}
	\begin{algorithmic}[1]
%		\algrestore{alg:p0}
		\State $PK, VK_N, \ms{share}$ $\leftarrow$ agree-on-key() \label{line:abe:agreeonkey}
%		\State Post \ms{PK} to blockchain % has well-defined interface, whereby writing triggers consensus => include in DKG ?
		\If{$p_i = \ms{proposer}$} \label{line:abe:ifproposer}
			\State{Generate and RB-Broadcast \ms{config}} \label{line:abe:rbconfig}
		\EndIf
		\Upon{RB-delivery of \ms{config}} \label{line:abe:uponrbdel}
		\State $v$ $\leftarrow$ valid-config(\ms{config}) ? $1$ : $0$ \label{line:abe:validconfig}
		\State Invoke $\ms{BIN\_CONS[config]}$.bin\_propose($v$) \label{line:abe:invokecons} % might need MVC for SMR? should converge relatively quickly
		\EndUpon
		\WUntil $\ms{bin\_decision} \neq \perp $ \EndWUntil
		\If {$\ms{bin\_decision} = 1$}
		\WUntil \ms{config} is RB-delivered \label{line:abe:waitrb} \EndWUntil
		\State \ms{ballot} $\leftarrow$ prepare-ballot(\ms{config, PK}) \label{line:abe:prepballot}
			\State $\ms{enc-ballots}$ $\leftarrow$ anon-vc(\ms{ballot}) \label{line:abe:encballots}
			\State $\ms{unique-ballots}$ $\leftarrow$ remove-duplicates(\ms{enc-ballots}) \label{line:abe:uniqueballots}
			\Return decrypt-ballots($\ms{unique-ballots}$) \EndReturn \label{line:abe:decballots}
		\Else
		\State Abort the election
		\EndIf
	\algstore{alg:election}
	\end{algorithmic}}
\end{algorithm}


==> evotingabfe/evoting-abfe.tex <==
\section{Arbitrary ballot elections} \label{sec:evoting:abfe}

In some situations, it is desirable for voters to be able to propose ballots that may comprise of diverse or otherwise arbitrary components. In the context of electing leaders or representatives, it can be useful to allow for write-in ballots, which allow voters to vote for a candidate without a priori agreement by $P$ to vote with respect to that individual, increasing flexibility. This holds true especially if the number of potential candidates is large (e.g. a population). If $P$ wish to exchange written opinions on some issue in a fair and robust manner, then an e-voting scheme that supports arbitrary ballot composition can be used directly.

%n such a scenario, voters may be compelled to consider only \textit{well-formed} ballots under some a priori agreed notion of well-formedness. 

To this end, we present an election protocol, Arbitrary Ballot Form Election (ABFE), that handles arbitrary ballot composition. Our scheme is \textit{robust}, and works in Anonymous Vector Consensus Protocol's model (c.f. Section~\ref{sec:model:model}). Furthermore, we attain \textit{public verifiability}, \textit{eligibility}, and \textit{non-reusability}. As we consider arbitrary ballots, we cannot rely on a clever mathematical construction to ensure the contents of individual ballots are not revealed. Similarly, we cannot rely on an election authority to maintain the secrecy of these ballots, as our protocol is decentralised. Nevertheless, we ensure that the contents of all ballots are hidden until the end of the election.

We proceed as follows. Firstly, we enumerate relevant cryptographic primitives. Then, we present the construction: an efficient electronic voting scheme that enables arbitrary ballot composition. Finally, we perform protocol analysis, verifying that the aforementioned properties are fulfilled, and present further discussion on the protocol.

\subsection{Building blocks}

To ensure that participants eventually obtain the same set of (correct) ballots and terminate the protocol in a deterministic fashion (or with high probability via randomization \cite{Mostefaoui2015}), it is necessary to invoke a primitive with the properties of Byzantine consensus. As such, we leverage our algorithm, Anonymous Vector Consensus Protocol (AVCP), presented in Section \ref{sec:avc:avc}. As suggested by its name, AVCP ensures that the identity of a voter is indistinguishable from that of all non-faulty voters, a consequence of AVC-Anonymity. Moreover, through traceable ring signatures, double voting is mitigated and eligibility requirements can be enforced, which follows from ARB-Validity.

With just AVCP, however, a participant's (unencrypted) vote is revealed immediately after it is broadcast to all parties. In such a situation, participants can alter their choice of vote based on the progress of the election, or indeed refuse to participate in the election, potentially preventing termination. Moreover, the contents of a ballot can reveal information about the voter to malicious parties, restricting and potentially denying their anonymity. Therefore, it is vital for ballot exchange to occur with encrypted ballots, which are then decrypted and revealed upon the termination of an instance of AVCP.

To this end, we leverage \textit{threshold encryption}, where processes who have access to a common (public) key can encrypt a message (ballot), requiring $k$ participants to collaborate to decrypt any message. In such a scheme, the collusion of up to $k - 1$ processes should result in no information about the contents of the ballot being revealed. Since AVCP is $t$-resilient when $t < \frac{n}{3}$, setting $k = t + 1$ maximises efficiency whilst retaining robustness. That is, by assumption, no ballots can be decrypted unless it is during the decryption phase of the protocol. We use Shoup and Gennaro's construction \cite{Shoup2002}, which is non-interactive, and so is appropriate for use over an asynchronous network, and can leverage the PKI - elliptic curve cryptography - typically used within distributed ledgers.

To agree on a common encryption key, we can either assume that the processes undergo a trusted setup, or that they perform distributed key generation (DKG). With the exception of \cite{Kate2012}, which is slightly esoteric in its network model and exposition, DKG typically relies on a synchrony assumption to ensure it executes in a cryptographically secure fashion \cite{Pedersen1991}, \cite{Gennaro2007}. Therefore, one can interchange a trusted setup or an appropriate DKG scheme in the following exposition, depending on their trust and network models.

Finally, we note that in an arbitrary ballot election, we can attempt to guarantee (in the boardroom model) that the contents of a ballot is revealed only at the end of the election without exploiting mathematical structure a la homomorphic tallying \cite{Cohen1985}. As such, a voter may be coerced into voting in a certain way, whose ballot could be identified by the coercer if some identifying contents that is unlikely to be generated by a normal voter is included in the ballot. Therefore, the scheme is best instantiated in an environment where external coercion is not a significant concern.

We present the protocol assuming no setup or strong PKI. We assume that processes in $P$ can instantiate pairwise reliable channels to communicate over, and each have a public key that identifies them uniquely. We also assume access to reliable, anonymous channels (which can be instantiated over Tor \cite{Dingledine2004}, for example), and that processes are aware of each other's public keys.

\subsection{Election protocol} \label{sec:evoting:abfeprotocol}
\subsubsection{State}
\input state.tex
Processes track various variables from the outset of the election. \ms{config} refers to a string that may contain rules of the election. For example, it may describe how the tallying procedure is to occur, which candidates voters may vote with respect to, the time-frame of the election, etc. We present the algorithm as if one proposer is generating \ms{config} - processes may alternatively use vector consensus to take some appropriate combination of proposed configurations. $PK, VK_N$ and $\ms{share}$ refer to parameters generated by distributed key generation or a trusted setup.  $\ms{bin\_decision} \in \{0, 1, \perp\}$ refers to the outcome of the instance of binary consensus $\ms{BIN\_CONS}[\ms{config}]$, and is initially set to $\perp$.

\subsubsection{Main algorithm}
\input election.tex
For encryption and subsequent decryption of ballots, processes partake in some distributed key generation scheme if keying material has not yet been agreed upon (i.e. if this is the first election for $P$ and a trusted setup is not assumed) (line \ref{line:abe:agreeonkey}). Then, to begin an election, process $p_i$, the proposer, generates a configuration (\ms{config}), which is reliably broadcast (lines \ref{line:abe:ifproposer} and \ref{line:abe:rbconfig}).

Assuming $p_i$ is non-faulty, all non-faulty processes will eventually RB-deliver \ms{config}. Then, processes pass \ms{config} to a deterministic validity function valid-config() (line \ref{line:abe:validconfig}), which is constructed in a similar manner to valid() in AVC (see Section \ref{sec:avc:avcprelim} for its characterisation). We defer further description of valid-config() to the discussion section. Based on the result $v \in \{0, 1\}$, processes propose $v$ in an instance of binary consensus (line \ref{line:abe:invokecons}).

Assuming processes agree to perform the election, processes first prepare their ballot locally (at line \ref{line:abe:prepballot}). The (unencrypted) ballot itself may be produced non-deterministically (i.e. depending on pre-defined rules, but otherwise arbitrarily). Then, a \textit{nonce} must be appended to their vote, in order to prevent voters from disrupting the election via a replay attack. Moreover, the ballot must be subsequently encrypted as per the threshold encryption scheme. Then, processes exchange ballots via anonymous vector consensus (at line \ref{line:abe:encballots}). We remark on the nature of this instance of AVCP:

Firstly, recall that, by AVC-Validity, that every value that is decided in a process' vector $V$ satisfies a pre-defined predicate valid(). In this election scheme, the validity predicate must, at minimum, ensure that encryptions are well-formed (i.e. valid() confirms that the ZKP embedded in an encrypted message is produced correctly).

Moreover, recall that all non-faulty processes propose 0 in all instances of binary consensus that they have not decided 1 in after $n - t$ 1's are decided (occurring at line \ref{line:avc:binpropzeros} of AVCP). Without an additional synchrony assumption, we must do this to ensure termination. In practice, however, it is often the case that much less than $t$ processes are faulty, and in the context of an election it is vital that one considers as many (correct) ballots as possible. As such, we can enforce that processes continue (potentially) proposing 1's for some pre-determined amount of time after $n - t$ 1's are decided, enabling all $n$ ballots to be decided in the good case. In some contexts, it makes sense to rely on such a synchrony assumption, especially if ballots are produced non-deterministically (i.e. at the whim of parties controlling particular processes).

Now, once AVCP has terminated, processes check for duplicate ciphertexts in \ms{enc-ballots} (line \ref{line:abe:uniqueballots}), removing any that are found. Importantly, processes must keep one copy of any duplicates found, so as to prevent a malicious process from nullifying an honest voter's ballot. Checking for duplicates is performed to prevent \textit{replay attacks}, i.e. malicious voters producing the same input as another process to attempt to skew the election result. Given that the domain of potential nonces is large enough, by the non-malleability of the encryption scheme, replay attacks are thwarted.

Then, all processes decrypt their ballots via threshold decryption, invoking the function at line \ref{line:abe:decballots}. Alternatively, processes may reconstruct the secret key corresponding to $PK$ via pooling shares if the secret is not to be used again or $P$ is to be changed. Such a decision is to be decided ahead of time (e.g. encoded in \ms{config}). Then, based on some a priori decided rule, ballots can be processed/summed appropriately.

We note that it is not necessary for a configuration to be decided immediately prior to an election if the election rules are known a priori. 

In the context of a replicated state machine tracking a distributed ledger, we can consider \ms{config} as comprising a block. In this context, it preferable to perform multivalued (or indeed vector) consensus to ensure total ordering of the blocks. For efficiency's sake, however, we present the protocol with respect to an instance of binary consensus.

We shall now describe how ballot decryption proceeds.


\subsubsection{Ballot decryption}
\input decryptbals.tex
Each process keeps track of four local variables, \ms{partial-decs}, \ms{buffered-decs}, \ms{ballots}, and \ms{has-broadcast} defined at lines \ref{line:dec:partialdecs}, \ref{line:dec:buffereddecs}, \ref{line:dec:ballots} and \ref{line:dec:hasbcastvar} respectively. The function partial-decryption() generates a partial decryption of an encrypted message, using a process' local share, as per the threshold encryption scheme. Similarly, combine-shares() combines $k$ valid partial decryptions of a given ciphertext to produce the associated plaintext.

Consider a non-faulty process $p$. $p$ inputs the vector of proposals decided from AVCP, all of which are well-formed encryptions of ballots. To this end, $p$ produces a partial decryption of each value (lines \ref{line:dec:foreach} and \ref{line:dec:partialinc}). $p$ then adds each (valid) partial decryption to their buffer \ms{buffered-decs} (lines \ref{line:dec:foreachownshare} and \ref{line:dec:addownshare}) and broadcasts their partial decryptions (line \ref{line:dec:bcast}). In doing so, $p$ sets $\ms{has-broadcast}$ to True (line \ref{line:dec:true}).

Since the threshold of recovery is $k = t + 1$, $p$ requires $t$ additional sets of valid partial decryptions to decrypt all ballots. So, upon receipt of a potential set of valid partial decryptions, $p$ verifies that the decryptions are exhaustive and well-formed (line \ref{line:dec:validdecs}). Given the validity of a set of partial decryptions, since other processes may progress faster, $p$ waits for $\ms{has-broadcast}$ to be True before buffering the valid partial decryptions (at line \ref{line:dec:incbuffer}) to ensure that all non-faulty processes broadcast their decryptions before combining shares locally. Then, once \ms{buffered-decs} contains enough shares for every ballot (fulfilling the predicate at line \ref{line:dec:enoughshares}), $p$ combines partial decryptions together as per the threshold encryption scheme (lines \ref{line:dec:foreachbuffered} and \ref{line:dec:combineshares}). Finally, $p$ returns the resulting (plaintext) ballots (line \ref{line:dec:return}).

%Ballot form TODO

%remark that config proposal could be voting on something more generally

%PID associated with a traceable ring signature / in consensus TODO

\subsection{Analysis and discussion} \label{sec:evoting:abeproof}
\subsubsection{Correctness} We prove correct each property that we claim holds in the election protocol. For simplicity, we assume that each process has the appropriate parameters corresponding to a common key stored locally (a share, the public key and the verification keys).

\underline{Robustness}: We assume that the proposer $p_i$ of \ms{config} is non-faulty. At line \ref{line:abe:rbconfig}, $p_i$ will RB-broadcast their configuration. By RB-Termination-1, all non-faulty processes will eventually RB-deliver \ms{config} (at line \ref{line:abe:uponrbdel} or \ref{line:abe:waitrb}). Further, by RB-Unicity, given that $p_i$ RB-broadcasts $\ms{config}$, only \ms{config} can be RB-delivered by non-faulty processes. Then, since valid-config() is deterministic, all non-faulty processes will output the same $v \in \{0, 1 \}$ (line \ref{line:abe:validconfig}), and propose $v$ in an instance of \ms{BIN\_CONS}. Then, by the intrusion-tolerance of binary consensus, no coalition of $t$ faulty processes can change the outcome of \ms{BIN\_CONS}. Then, by BBC-Agreement, BBC-Termination, and BBC-Validity, all non-faulty processes will eventually decide $v$.

Suppose then that $v = 1$, i.e. the election proceeds. Then, RB-Termination-1 guarantees that processes will eventually RB-deliver \ms{config} if not yet done (at line \ref{line:abe:waitrb}). As at most $t$ processes might be faulty, i.e. might not behave correctly in \ms{anon-vc} (at line \ref{line:abe:encballots}), $n - t$ non-faulty processes will. By AVC-Validity, every encrypted ballot decided will fulfil the validity predicate valid(),  ensuring that all encryptions are well-formed. % security of enc scheme?

Then, by AVC-Validity, AVC-Termination and AVC-Agreement, all non-faulty processes will eventually decide on $\geq n - t$ valid, encrypted ballots. After discarding duplicates (at line \ref{line:abe:uniqueballots}), processes will begin ballot decryption, invoking the function at line \ref{line:abe:decballots}. There, each non-faulty process, for which there are $\geq n - t$ of, will produce the partial decryption for each unique vote that was decided, which is then broadcast (at line \ref{line:dec:bcast}). Eventually, all non-faulty processes will eventually receive $k - 1 = t < n - t$ valid partial decryptions, which they can perform combine-shares() on for each value decided in AVCP (at line \ref{line:dec:combineshares}), which produces the same output (even if different, but still valid share decryptions are used by different processes). Consequently, all non-faulty processes will return the same vector $\ms{ballots}$.

Finally, we note the following:
\begin{itemize}
	\item The threshold encryption scheme \cite{Shoup2002} is non-malleable. % CCA security => non-malleability?
	\item With high probability, no two valid signatures will look identical due to the randomness intrinsic to signing (c.f. Lemma \ref{avc-labelling} in the proof of AVCP's correctness).
	\item With high probability, two voters who produce the same (unencrypted), with the exception of the nonce, will produce different ballots, given that the domain of potential nonce values is large enough.
\end{itemize}
It follows that no coalition of processes of size $t$ or less can produce a conflicting, but valid, ciphertext that will render an honest process' vote nullified in the check at line \ref{line:abe:uniqueballots}, and that no two honest process' will unintentionally produce the same ciphertext.

\underline{Public verifiability}: By robustness, all non-faulty processes will return the same vector \ms{ballots}. Then, any third party can ask for \ms{ballots} from the processes in $P$. On receipt of $t + 1$ identical vectors \ms{ballots}, a party can be sure, given that up to $t$ processes are faulty, that the vector corresponds exactly to the agreed upon outcome of the election.

\underline{Weak privacy}: All non-faulty processes will propose an encrypted ballot in anon-vc (AVCP), with the threshold for decryption set to $k = t + 1$. Then, since up to $t$ processes may collude, and by the correctness of the threshold encryption scheme, it follows that combining $t$ shares together reveals no novel information about the nature of the encrypted message. Consequently, no messages will be decrypted prior to the invocation of decrypt-ballots(), completing the proof.

\underline{Eligibility}: In all stages of ARBP bar the sending and receiving of \INIT \ messages, and at all subsequent times, processes only process input from processes in $P$ by (implicit) assumption. Then, by the unforgeability of the traceable ring signatures used in ARBP, no process outside of $P$ can produce a signature that associates them with the ring $P$.

\underline{Non-reusability}: Processes propose their votes by AVCP only through the ARB-broadcast of a value. So, by ARB-Unicity, no non-faulty process will ARB-deliver more than one value from a particular process, and by the $t$-resilience of AVCP, at most one value proposed by a non-faulty process will be decided.

Thus, we have shown that all relevant properties of the voting scheme hold.

\subsubsection{Discussion}

\underline{The function valid-config()}:
As described, the process valid-config() disseminates a ``valid'' configuration for bootstrapping an election. This kind of validity is application-specific. One reasonable rule to include is that the pool of potential candidates to vote on, if to be limited, must be non-trivial, i.e. contains at least two candidates. Another rule could be to ensure that the ``threshold'' by which a candidate wins is set fairly, i.e. is roughly a majority. To enforce these kinds of rules, the \ms{config} would have to be produced in a particular, known encoding, such as JSON.

\underline{Receipt-freeness}:
One way that an adversary can generate a receipt is through deliberately double-signing with the traceable ring signatures that we make use of in the scheme. One interesting way around this was proposed in \cite{Chow2008}, suggesting the use of escrowed linkable ring signatures through an election authority, making the adversary unable to determine whether it was the authority or the voter who produced the double-sign. However, we do not make use of trusted third parties per se, and so we cannot employ such a technique. Moreover, this does not prevent processes from revealing the randomness they used to encrypt their ballot to generate a receipt.

\underline{Decryption optimisation}:
We note that we only require $2t$ processes to broadcast their partial decryptions (at line \ref{line:dec:bcast}), since a non-faulty process needs $t$ additional partial decryptions to perform ballot decryption. Given processes are indexed consistently, we can require the first $2t$ processes to broadcast their partial decryptions. This results in less messages being sent overall, but may not speed up termination, depending on the topology of the network.


==> oldintro.tex <==
%\vincent{Motivations could rely on Frontrun.me and Governance: \url{https://blog.goodaudience.com/blockchain-governance-101-eea5201d7992}}

\iffalse  %CC: if-intro: current
%Blockchain promises to distribute decision power, or \emph{governance}, over a group of participating machines.
Permissionless blockchains have become a popular paradigm to track asset ownership or run 
distributed applications in an open environment accessible to any Internet users.
Yet, as of today its governance is usually externalized to independent and often fragmented fundations. Instead of being upgradable, blockchain protocols multiply through forks like for ETH vs. ETC or create conflicting situations like the recent divergence of opinions around Bitcoin Cash (BCH) and Satoshi's Vision (BSV). 
Instead, the blockchain should ideally rely on its participants to
%To select the participants that can 
decide of the future of itself.
%, blockchains
%%Permissionless blockchains typically 
%use complex mechanisms. 
Permissionless blockchains require its deciders to consume
%with Sybil attacks~\cite{Douceur2002} by consuming 
%Permissionless blockchains typically cope with Sybil attacks~\cite{Douceur2002}, these mechanisms usually consume 
a large amount of resources, which is not sustainable at large scale.
The consortium blockchain alternative requires its set of deciders to be predetermined~\cite{Buterin2015}. An interesting alternative is the community blockchain~\cite{Vizier2018} that 
allows different sets of nodes, or \emph{communities}, to decide at different times. % but does not detail the selection of deciders.
%A popular alternative is to allow a subset of permissioned nodes to propose new blocks.
%While consortium blockchains require this set to be predetermined~\cite{Buterin2015}, a recent alternative, called community blockchains~\cite{Vizier2018}, allow different sets of nodes, or \emph{communities}, to decide upon different blocks over time. 

By failing to account for the opinions of all participants, the governance of blockchain cannot be democratic.
A first idea is to choose a representative community by drawing public keys at random and hoping that they are owned by the right number of blockchain participants~\cite{Gilad2017}.
%New blockchain protocols are continuously introduced rather than being replaced (e.g., ETH and ETC). 
%Another approach is for participants to invoke a replicated function that is typically agnostic to the system participants and may fail to output a reasonably sized community. 
If the community is too large, reaching consensus could be too slow. If the community is too small, malicious participants could feasibly coerce sufficiently many community members in order to steal assets.
%In traditional blockchains, the node that is the fastest to solve a crypto puzzle is more likely to impose its block decision.
A second approach is to have one leading participant imposing its decision \cite{Castro1999}. 
%which risks the introduction of bias. 
This leader could be 
%This leader, a single point of failure, could be 
tempted to either include his preferred participants as if it was returning a service to his friends, or to expect a favour from the community members in return for their selection.

\else %CC: if-intro: alternative

Blockchain technology promises to distribute decision power over a group of
participants and is often used to run distributed computations in an open
environment or to track valuable items in applications accessible to any
Internet user.  Yet, the so-called \emph{permissionless} blockchains like
Bitcoin or Ethereum suffer from heavy computational effort and from
external, inefficient governance models, because decisons about the
protocols themselves are relegated to an external, human level.  Multiple
recent forks in those systems demonstrate this.

The alternative model of a \emph{consortium blockchain} relies on a set of
predetermined decision makers, which can be upgraded through the protocol
over time.  Another model is the community blockchain~\cite{Vizier2018}
that allows different sets of nodes, or \emph{communities}, to decide at
different times.  Such blockchains have also been called
\emph{permissioned}.  They operate much faster than permissionless
protocols and do not rely on costly computations for decision making.

This paper addresses the problem of voting and governance in permissioned
blockchains such that the opinion of every participant is accounted for.
In accordance with established election protocols, voting procedures, and
other decision-making rules, we demand a level of anonymity to protect the
voters.
%
\fi %CC: if-intro: end
%
Our contribution is called \emph{\name}, a mechanism where blockchain participants express their individual opinion through ballots, containing application-specific and otherwise arbitrary contents, to reach a collective decision regarding a representative community. More precisely, we present a protocol with the following properties:
%The idea adapts the concept of electronic boardroom voting, where participants act both as voters and talliers,
\begin{enumerate}
\item {\bf Secrecy and voter indistinguishability.} For governance, it is crucial for participants to elect freely their representatives without being influenced by other participants. 
For this reason, we cannot rely solely on point-to-point channels that would expose the participants identity to each other when exchanging ballots.
%If processes were to exchange (arbitrary) ballots over reliable channels, their identities would be inextricably associated with each other. %enabling potential profiling and punishment.
%This is why a crypthographic technique is needed to guarantee ballot secrecy during the vote.

\item {\bf Fraud detection.} Voter indistinguishability could be leveraged by malicious participants to influence the vote and steal assets in blockchains. It is thus important to detect a duplicate vote coming from a participant to ensure that the election is democratic and to identify the issuer of this duplicated vote. %, which is easy enough to detect with point-to-point channels. 
%However, processes can neither be sure of who has voted nor how many times each process has voted, and so an additional mechanism is needed.

\item {\bf Robustness.} In the blockchain context that aims at tracking ownership of digital assets, protocols should tolerate the presence of malicious behaviors, often expressed as Byzantine failures.
In particular, a resilience optimal consensus is known to be reachable when up to $t < \frac{n}{3}$ Byzantine failures can occur among $n$ participants.  
%In particular tolerating up to $t < \frac{n}{3}$ Byzantine failures among $n$ participants 
%$n$ participants must reach consensus on a block despite the presence of up to a third of $t < \frac{n}{3}$ of Byzantine participants communicating over the Internet where communication is not synchronous.

\item {\bf Write-in ballots.} The ballot should be generic to allow participants to propose votes outside of a list of pre-established candidates
%to suggest new proposal 
through the use of 
 \textit{write-in} ballots. 
% containing votes outside of a list of pre-established candidates. 
This precludes homomorphic encryption solutions~\cite{Cramer1997}, whose zero-knowledge proofs and ballot encoding techniques become prohibitively expensive at scale.

\item {\bf Peer-to-peer.} A voter should be  able to be a vote tallier as the participants that offer a blockchain service are also the ones that benefit from it. 
	This precludes solutions based on mixnets~\cite{Golle2004}, public bulletin boards \cite{Groth2004}, and those with escrowed cryptography, like linkable ring signatures~\cite{Chow2008}, all of which require the set of talliers to be disjoint to the set of voters.

\end{enumerate}

%If processes were to exchange (arbitrary) ballots over reliable channels, their identities would be inextricably associated with each other, enabling potential profiling and punishment. Naively, sending ballots over anonymous channels may resolve this problem. However, without additional machinery, processes can neither be sure of who has voted nor how many times each process has voted. 



%\item {\bf Attack resilience.}
%For blockchain participants to reach consensus on a unique block at a given index, one must assume less than a third of participants are Byzantine~\cite{}, which limits the size of a coalition to $\frac{n}{3}$.
%In particular, secure election schemes, like homomorphic encryption support ubiquitous ballot secrecy but sacrifices ballot flexibility which make them badly suited to the blockchain model.

%\item {\bf 1/3-fault tolerance and no synchrony.}
%For blockchain participants to reach consensus on a unique block at a given index, one must assume less than a third of participants are Byzantine.
%In this environment where a majority of processes are assumed to be trustworthy for correctness, or where the threat of coercion is small, sacrificing some level of ballot privacy to support arbitrary ballot composition can be of benefit.
%In particular, secure election schemes, like homomorphic encryption support ubiquitous ballot secrecy but sacrifices ballot flexibility which make them badly suited to the blockchain model.
%Because blockchain community can be very large, encoding the candidate choices mathematically may be prohibitively expensive and certainly requires a priori agreement.
%\vincent{The reason being that homomorphic encryption is that as far as we know it does not scale, as it requires vote for $k$ participants in $k$ individual instances.}
%In comparison, our approach supports arbitrary ballot composition that supports write-in ballots, allowing for flexible and potentially ad-hoc elections. 
%\vincent{(Another approach is using mixnet, but it always relies, as far as we know, on a set of authorities (taliers) and voters to be different)}
% 	The DC net would require $O(k)$ message delays due to $k$ subsequent rounds of broadcast (one for each voters). % (we do not know whether it is Byzantine fault tolerant or partially synchronous).
%	In our case, the communication complexity is $O(cn^4)$ where $c$ is the size in bits of the used key (typically 256 bits).
%	
%	There is a solution with linkable ring signatures but they require the set of taliers to be disjoint from the set of voters.

%\item{\bf Single-user but anonymous ballot.}
%\vincent{vector consensus.}
%If processes were to exchange (arbitrary) ballots over reliable channels, their identities would be inextricably associated with each other, enabling potential profiling and punishment. Naively, sending ballots over anonymous channels may resolve this problem. However, without additional machinery, processes can neither be sure of who has voted nor how many times each process has voted. 

%	\vincent{Our ingredient:} 
To offer an electronic voting scheme that offer these properties, we combine threshold encryption~\cite{DDF94}, traceable ring signatures~\cite{Fujisaki2007} and Byzantine consensus~\cite{LSP82} in the following way.
First, we leverage \textit{threshold encryption}~\cite{DDF94, Desmedt1992}, ensuring that no malicious coalition of size $t<\frac{n}{3}$ or less can decrypt any message, making our solution \textbf{robust} to Byzantine failures while offering {\bf secrecy} by revealing the tally only after the vote concluded.
\textbf{Voter indistinguishability} is achieved through minimal anonymous message passing, requiring a single anonymous broadcast from each voter.
Second, we leverage \textit{traceable ring signatures}~\cite{Fujisaki2007} that enable processes to prove their membership from any given set of processes without revealing their identity, yet exposing the signer identity only if they sign two different messages.
Third, we introduce an anonymous variant of the vector consensus problem~\cite{DS98} with no restriction on the proposed \textbf{write-in ballots} and solve it using a new anonymous solution to the reliable broadcast, making our solution strictly \textbf{peer-to-peer}.

%% This traceability guarantees {\bf fraud detection} to prevents double signing, by exposing the identity of the signer only if they sign two different messages. 
% As such, this {\bf fraud detection} held processes accountable for their misbehaviour.
%
% that is resilience optimal and converges in three message steps.
%
%%To solve this problem, 
%we leverage \textit{traceable ring signatures}~\cite{Fujisaki2007} that enable processes to prove their membership from any given set of processes without revealing their identity, yet exposing the signer identity only if they sign two different messages.
%% This traceability guarantees {\bf fraud detection} to prevents double signing, by exposing the identity of the signer only if they sign two different messages. 
% As such, this {\bf fraud detection} held processes accountable for their misbehaviour.
% \textbf{Voter indistinguishability} is achieved through minimal anonymous message passing, requiring a single anonymous broadcast from each voter. We ensure {\bf secrecy}, in that the tally is only revealed after voting has concluded, preventing voters from deciding how, or if, to vote depending on the partial tally. To this end, we leverage \textit{threshold encryption}, ensuring that no malicious coalition of size $t<\frac{n}{3}$ or less can decrypt any message, making our solution
%% Moreover, our solution is 
%\textbf{robust} to Byzantine failures. is strictly \textbf{peer-to-peer} and supports \textbf{write-in ballots} as it relies on consensus, which places no essential restriction on the proposed values.
	
%	\vincent{Ingredient lists: %Anonymous reliable broadcast \superseteq 
%	Application of traceable (accountability) ring signature to cope with denial of service attack by blacklisting the originator of the duplicated votes + reduction to binary consensus}
		
%\end{itemize}
%\textbf{Contribution and Roadmap}:

Finally, we believe our solution is practical for three reasons. First, our extension of reliable broadcast to Anonymous Reliable Broadcast Protocol (ARBP) converges in three message steps and require $O(n^3)$ messages.
Second, our Anonymous Vector Consensus Protocol (AVCP) that solves the new problem of \textit{anonymous vector consensus} requires $O(n^4)$ messages and can converge in four message steps in the good case.
Both ARBP and AVCP handle $t < \frac{n}{3}$ Byzantine-faulty processes.
%
%We propose two protocols that can be used as building blocks in other distributed systems. Both protocols provide \textit{anonymity}, where a process' proposal is indistinguishable from that of all other honest processes. Firstly, we extend reliable broadcast to Anonymous Reliable Broadcast (ARB), which converges in three message steps and handles $t < \frac{n}{3}$ Byzantine-faulty processes, which is $t$-optimal.  Secondly, we extend the definition of vector consensus to \textit{anonymous vector consensus}, and present a protocol, Anonymous Vector Consensus Protocol (AVCP), that implements it. 
%
%Our proposed solution is $t$-optimal, efficient in that it may converge in four message steps in the good case, and round-optimal.  In terms of message complexity, our protocols are efficient ($O(n^3)$ for all-to-all ARB and $O(n^4)$ in the worst-case for AVCP).
%Using these primitives, we present a $t$-resilient electronic voting scheme that supports arbitrary ballots that forms the basis of \name. 
Third, we evaluate empirically both the cryptographic primitives we rely upon, and the distributed protocols we have devised. For an arbitrary ballot election with $n = 100$ participants, our protocol converges in less than 10 seconds.

%\textbf{Related work}



==> state.tex <==
\begin{algorithm}[htp]
\label{alg:state}
{\small
\caption{Election state}
	% state in pseudo-code
	\begin{algorithmic}
		\State $config$ \Comment{Application-specific configuration proposal, initially $\perp$}
		\State $PK, VK_N$ \Comment{The public key and verification keys produced by DKG or a trusted dealer}
		\State $share$ \Comment{A share of the secret key produced via DKG or a dealer}
		\State $\ms{enc-ballots[1..n]}$ \Comment{An array storing the result of ballot exchange via AVC}
		\State $\ms{bin\_decision} \leftarrow \perp$ \Comment{Binary decision corresponding to an instance of binary consensus}
	\end{algorithmic}}
\end{algorithm}

